Practically and Theoretically Efficient Garbage Collection for Multiversioning

Multiversioning is widely used in databases, transactional memory, and concurrent data structures. It can be used to support read-only transactions that appear atomic in the presence of concurrent update operations. Any system that maintains multiple versions of each object needs a way of efficiently reclaiming them. We experimentally compare various existing reclamation techniques by applying them to a multiversion tree and a multiversion hash table. Using insights from these experiments, we develop two new multiversion garbage collection (MVGC) techniques. These techniques use two novel concurrent version list data structures. Our experimental evaluation shows that our fastest technique is competitive with the fastest existing MVGC techniques, while using significantly less space on some workloads. Our new techniques provide strong theoretical bounds, especially on space usage. These bounds ensure that the schemes have consistent performance, avoiding the very high worst-case space usage of other techniques.

==> artifact-instructions.tex <==
\appendix
%
\section{Artifact Evaluation Appendix}
\label{sec:ae}

\subsection{Abstract}

\Hao{place holder - still need to be updated}
This artifact contains the source code and scripts to reproduce all the graphs and tables in Section \ref{sec:experiments}.

\subsection{Artifact check-list (meta-information)}

\begin{itemize}
	\item \textbf{Algorithm:} all the algorithms from Figure \ref{fig:exp}
	\item \textbf{Program:} microbenchmarks
	\item \textbf{Compilation:} OpenJDK 11.0.9.1
	\item \textbf{Binary:} binary not included
	\item \textbf{Run-time environment:} Ubuntu 16.04.6 LTS
	\item \textbf{Hardware:} any multi-core machine with at least 60 GB main memory.
	\item \textbf{Output:} graphs from Section \ref{sec:exp} as PNG files.
	\item \textbf{Experiments workflow:} one script for compiling the experiments and one script for generating all the graphs.
	\item \textbf{Disk space required (approximately):} 46 MB
	\item \textbf{Time needed to prepare workflow:} approximately 10 minutes
	\item \textbf{Time needed to complete experiments:} approximately 20 hours
	\item \textbf{Publicly available:} yes
	\item \textbf{Code licenses:} MIT License
\end{itemize}

\subsection{Description}

\subsubsection{How delivered}

Available as open source under the MIT software license: \url{https://github.com/yuanhaow/vcaslib}.

\subsubsection{Hardware dependencies}

To accurately reproduce our experimental results, a multi-core machine with at least 300 GB of main memory is recommended. When using less than 300 GB, you may see some small overhead due to Java's garbage collector running more frequently. At least 60 GB of main memory is required to run the PNB-BST in Figure \ref{fig:exp} because it never garbage collects nodes.

\subsubsection{Software dependencies}

Our artifact is expected to run correctly under a variety of Linux x86\_64 distributions. Our Java experiments require OpenJDK 11 and our C++ experiments were compiled using g++ 9.
For scalable memory allocation in C++, we used jemalloc 5.2.1  (\url{https://github.com/jemalloc/jemalloc/releases/download/5.2.1/jemalloc-5.2.1.tar.bz2}).
Our scripts for running experiments and drawing graphs require a Python 3 installation with mathplotlib.
We used the \texttt{numactl} command to evenly interleave memory across the NUMA nodes.

\subsubsection{Data sets}

None.

\subsection{Installation}

Source code can be complied by running \texttt{./compile\_all.sh}.

\subsection{Experiment workflow}

After compiling, run \texttt{./generate\_graphs\_from\_paper.sh}  to generate all the graphs and store them in the \texttt{graphs/} directory.

\subsection{Evaluation and expected results}

On a machine with 140 or more logical cores, the results should be very similar to those reported in this paper. 
Figures \ref{fig:exp}i and \ref{fig:exp-cpp}c require at least 72 logical cores to reproduce.

\subsection{Experiment customization}

For instructions on how to customize the number of threads, workload, range query size, and data structure size in each experiment, please see the README file in the GitHub repository (\url{https://github.com/yuanhaow/vcaslib}).

\subsection{Notes}

None.

\subsection{Methodology}
Submission, reviewing and badging methodology:
\begin{itemize}
	\item \url{https://ctuning.org/ae/submission-20190109.html}
	\item \url{https://ctuning.org/ae/reviewing-20190109.html}
	\item \url{https://www.acm.org/publications/policies/artifact-review-badging}
\end{itemize}

==> hashtable-figures.tex <==


%\begin{figure*}
%	\hspace*{-.6in}
%	\includegraphics[width=1.05\linewidth,trim=0 0 0 2cm, clip]{graphs/hashtable-vary-rqsize-100K-60-60-60-uniform-oversubscribed.png}
%	\caption{Hashtable initialized with 100K keys, 60up-60srt-60rt, oversubscribed, uniform}
%	\label{fig:hashtable-100K-oversub}
%\end{figure*}

==> implementations.tex <==
% !TEX root =  main.tex

\section{Implementations and Optimizations}
\label{sec:implem}

We show how to use the singly- and doubly-linked list algorithms in the previous sections to improve two existing MVGC techniques (steam and BBF+) as well as develop a new one.

\subsection{Lock-free Steam}

%Steam works in transactional system, where each thread manages a disjoint set of transactions.
%Each thread $p$ keeps track of the timestamps of the transactions it manages in a local list
%and announces the current timestamp 
In Steam~\cite{bottcher2019scalable}, version lists are singly-linked lists, maintained sorted, in decreasing order, 
based on the timestamps of the versions.
A new version is added in the version list of an object, every time the object is updated. 
Right after, $p$ traverses the version list that it has just updated, 
and compacts it, by deleting from it all versions that are not needed by any currently active transaction. 
To implement compaction, the announced timestamps (by active transactions) are collected and
and sorted, in decreasing order, by $p$ before starting the traversal of an updated version list. 
Transactions in Steam use locks to apply multiple updates in an atomic way. 
Compaction of version lists is piggy-backed in transactions' processing 
(as part of objects' updates), thus a version list is locked 
when its compaction takes place. 
It follows that Steam is blocking. 

Given that compaction of a version list is performed every time 
a new version is added in it and assuming that announced timestamps are collected every time
a compaction occurs, the size of any version list is $O(P)$ (recall that $P$ is the number of processes).
We have implemented a lock-free version of Steam, called \texttt{SteamLF}, 
by employing the lock-free compaction algorithm presented in Section~\ref{sec:sll}. 
Specifically, \texttt{SteamLF} implements and manipulates each version list using the 
lock-free singly-linked list implementations presented in Figure~\ref{alg:singly-linked-list-compact}. 
Apart from this change, \texttt{SteamLF} works in the same way as Steam. 
Invariant~\ref{} implies that \texttt{SteamLF} maintains the $O(P)$ space bound of Steam. 

\here{PF: If the space bound of ssl does not hold, we need to update the last sentence above.
It seems to me that the bound is tighter than O(P), it is O(\# of needed versions).}

\here{PF: collect versus scan versus list traverse?}

\ignore{
\begin{itemize}

	\item Recall that Steam compacts a version list whenever a new version is added to it.
	\item The original Steam paper locks the version list before compacting, we can make this lock-free using our lock-free compact from Section~\ref{sec:sll}. We call the resulting algorithm \texttt{SteamLF}.
	\item If the announcement array is scanned on every compact, then this would maintain the space bounds of Steam (i.e. each version list has length at most $O(P)$).
\end{itemize}
}

\subsection{Practical BBF+}
\label{sec:pBBF+}

We propose a more practical version of BBF+, called PBBF+, 
which employs RangeTracker~\cite{BBF+21}, the linerizable implementation of a range-tracking object used by BBF+, 
but replaces the doubly-linked list implementation of BBF+
with the doubly-linked list implementation described in Section~\ref{sec:dll}. 
We provide more details below, starting with a description of  RangeTracker.
%
%We first provide a more detailed description of RangeTracker. 

%{\em RangeTracker}. 
A range-tracking object supports three operations, 1) \announce\ to announce a new timestamp, 2) \unannounce\ 
to declare that a previous announcement is no longer active, and 3) \deprecate, which 
declares that a version $v$ of an object is no longer the object's current version and 
identifies a set of unneeded nodes that can be safely disconnected from the object's version list.   
Every time a version $v$ ceases from being the current, 
\deprecate\ is invoked to declare that $v$ is no longer current and compact the version list $v$ resides. 

RangeTracker ensures that, in the worst case, \announce\ and \unannounce\ take $O(1)$ steps, 
and \deprecate\ takes $O(P\log P)$ steps but its amortized step complexity is $O(1)$. 
Operations \announce\ and \unannounce\ use a destination object~\cite{BW20a} to announce and unannounce 
timestamps in an announcement array $Ann$ in $O(1)$ steps.
To achieve its bounds, operation \deprecate\ works as follows. 
When a thread $p$
calls \deprecate\ for some version $v$, $v$ is appended in a local list where $p$ stores
objects it has deprecated; the list is sorted in decreasing order of timestamps of the deprecated objects it contains. 
If the size of $p$'s local list becomes $P\log P$ (where $P$ is the number of processes), a {\em flush phase} is performed: 
$p$'s  list is appended in a shared queue $Q$ containing such lists; then, two lists are extracted from $Q$,
their contents are merged and they are compared against a sorted version of $Ann$ to determine those versions
that are still needed, which are appended again into $Q$, and the set of the unneeded nodes that will be returned. 
This process is done with care, so that a flush phase requires $O(P\log P)$ steps and is perfrormed once
for every $O(P\log P)$ calls to \deprecate. Moreover, it is proved in~\cite{BW20a},
that RangeTracker satisfies the space bound of $O(H + P^2\log P)$, where $H$ is the number of needed versions. 

\y{
Experiments showed that employing RangeTracker results in some space overhead in practice. To reduce constants
in the space bound it ensures, we have implemented the following optimizations:
\begin{itemize}
\item pop a constant number of queues bigger than two every time we execute the flush phase. \here{PF: Have we implemeneted this optimization? Is it worth-mentioning?}
\Hao{I think this is worth mentioning, I wrote some more details about it in Section~\ref{sec:opt-notes}}
\item before we push a local queue in the global queue, compact the list, i.e., try to remove those versions in it that are already identified as unneeded. 
These techniques may reduce the space overhead imposed by RangeTracker without violating the space and time bounds it ensures. \Hao{This turned out to be a key optimization in reducing space usage in the tree data structure. (The details as to why should probably go in the experiments section.)}
\end{itemize}

Another optimization we have discussed is to ocassionally, pick a random version list to go through and compact. 
Have we tried this? Shall we refer to it?
}
\Hao{I tried it a long time ago and it did not seem to help at the time. I have not tried it with the current code which has changed significantly.}

{\em Lock-Free Doubly-Linked List}. We first present some of the details of TreeLL,
as it served as the starting point for designing DLL. We mainly focus on the implementation 
of \remove, as the rest of the routines are much simpler and do not impose any major difficulties.
%BBF+-DLL (as DLL) supports the operations, \tryAppend, which appends a node at the
%head of the list, \find, which searches for the first node in the list that has a timestamp 
%smaller than or equal to its argument, and \remove, which takes a pointer to a node as an argument 
%and splices the node out from the list. 
TreeLL supports the operations, \tryAppend, \find, and \remove, which have similar
functionality as the corresponding operations of DLL (the implementation in Section~\ref{sec:dll}). 
To remove a node, TreeLL marks it for deletion and then splices it out from the list. 
The major drives behind the design of \remove\ in PPB+-DLL are to avoid
list inconsistencies when deleting subsequent nodes, while ensuring 
the desired theoretical bounds.

TreeLL embeds a conceptual priority tree in the linked list
whose inorder traversal results in an ordered sequence of the list nodes.
TreeLL owns its name to this technique of organizing removals based on a priority tree.
%(this idea has been proposed in~\cite{++} for parallel list contraction). 
As long as deletions take place at the leaves of the tree (i.e., as long as 
a node is deleted only after all its descendants in the tree have been deleted), 
no two subsequent nodes of the tree are deleted concurrently, so 
consistency is ensured. However, some leaves may be still needed for answering queries.
Such leaves may block progress of removals and result in higher space bounds. 
To solve this problem, PBF+-DLL uses a helping mechanism 
which allows marked nodes that may have an unmarked neighbor to be spliced out (in some cases). 
This is done with much care, using two special helping routines, namely \spliceUnmarkedLeft, and \spliceUnmarkedRight, 
which ensure that consistency of the list is maintained. Moreover, this design 
preserves the desired bounds. 
Specifically, TreeLL ensures that 
at most  $2(L-R) + O(P\log L_{max})$ nodes remain in the version lists in an execution
containing a total of $L$ appends and $R$ removes, and at most $L_{max}$ appends 
on a single version list. It also ensures that 
\tryAppend\ and \getHead\ 
take $O(1)$ steps, and the amortized  number of steps for \remove\ is $O(1)$.

\spliceUnmarkedLeft\ and \spliceUnmarkedRight\ are pretty complicated, and  
experiments illustrated that they are pretty heavy in terms of performance. 
To come up with DLL, we first tried deactivating 
\texttt{spliceUmarkedLeft} and \texttt{spliceUnmarkedRight}, thus compromising
the space bound that TreeLL exhibits. 
Unfortunately, experiments showed that this simple solution ended up increasing 
space usage significantly (resulting in version lists that were on average twice 
as long as needed). DLL is thus a new proposed design, which avoids this space cost,
maintaining the good space bounds from~\cite{BBF+21}\here{PF: Is the space bound
the same for both DLL algorithms, the one in Section~\ref{sec:DLL} and TreeLL?}. 

\here{PF: We need to say more here.}
In terms of time, DLL ensures that \tryAppend\ and \getHead\ 
maintain the $O(1)$ bound of TreeLL, but the amortized  number of steps for \remove\ is $O(c)$,
where $c$ is the number of concurrent removals of consecutive nodes in the list.
Experiments showed that $c$ is usually a small constant; specifically, 
we saw that each \remove\ visits less than $3.6$ nodes on average \here{PF: Hao, please check if this number
is correct.}. This implies that, from a practical perspective, relaxing the time bound for \remove\
to $O(c)$ is a good compromise. 

\begin{theorem}

\end{theorem}


%Next, we tried a more practically efficient doubly linked list algorithm (without the theoretical guarantees of the one presented in the DISC paper) shown in Algorithm~\ref{alg:doubly-linked-list}, and that speed things up a little bit.


\ignore{

\paragraph{{\em \bf BBF+.}}
We start by providing an overview of BBF+. 
BBF+ assumes that every query sets a timestamp (i.e., it records an increasing integer in a global shared variable) 
at the beginning of its execution. Every update operation starts by reading the current timestamp 
(stored in this global variable) and uses it to stamp all the updates it performs. The previous value 
of an updated object (and its timestamp) are appended in the object's version list. 
After setting a new timestamp, a process executing a query proceeds to read the objects
that are necessary for computing its response. To do so in a consistent way, 
it traverses the version list of each such object and collects the first version it finds there 
with a timestamp that is smaller than or equal to the timestamp that the query set. 

Garbage collection in BBF+ employs the following two major components: 1) a {\em range tracking object},
which stores a set of versions and identifies those that are no longer needed, and 
2) a lock-free {\em doubly-linked list} to implement each object's version list, 
which supports an operation \Remove\ for disconnecting the unneeded versions. 
We briefly discuss each of these mechanisms below.

\paragraph{{\em \bf Practical Version of BBF+.}}
}


\subsection{SPAA2}
\Hao{TODO: pick better names for our algorithms.}

SSL-MVGC

\begin{itemize}
	\item A combination of BBF+ and SteamLF. The high-level idea is to use the range tracker from BBF+ to identify version lists with garbage in them, and then compact any version list that is returned by the range tracker.
	\item This allows us to use a singly linked list, which saves space (no need for back pointers), and time, but the disadvantage is having to re-traverse from the head when removing nodes.
	\item  More precise description of algorithm: if $h_{o}$ is the current head of a version list $L$, whenever we append a new head $h_{n}$ to $L$, we \texttt{deprecate} the triplet $(L, h_{o}.ts, h_{n}.ts)$, where $[h_{o}.ts, h_{n}.ts)$ defines an interval of time. 
	This \texttt{deprecate} operation returns a (possibly empty) list of previously deprecated triplets who's time intervals are no longer reserved. We call \texttt{compact} on each version list in the triplets that are returned. Note that a version list could be \texttt{deprecate}d multiple times, each time associated with a different time interval, so we remove duplicates before calling compact.
	\item If a triplet $(L, h_{o}.ts, h_{n}.ts)$ is returned by \texttt{deprecate} and later \texttt{compact(L)} is called, then $h_{o}$ is guaranteed to not be reachable in $L$ and will never become reachable again. Note that $h_{o}$ might have been removed by some earlier compact on $L$, so this call to \texttt{compact(L)} might end up finding no nodes to remove.
	\item Brief justification of why space bounds of BBF+ are maintained.
	\item Theoretical time bounds can be bad if version lists get long.
	\item TODO (Hao): finalize the set of optimization in the experiments and describe them here
\end{itemize}


Finally, we tried making the linked lists singly linked (further weakening its theoretical guarantees), and this had the best throughput out of all these variations (while at the same time maintaining the low space overhead of the original algorithm).
Since we no longer maintain back pointers, deleting from the middle of the list requires re-traversing the list from the head pointer.
This turns out to not be that expensive in our experiments because the version lists tend to be short.
The high-level idea behind this algorithm is to use our range tracker to identify version lists with garbage in them, and then scan\&compact any version list that is returned by the range tracker.



\ignore{
\noindent 
{\bf Memory Reclamation for nodes deleted from version lists.} 
As soon as a node is sliced out from a version list, it can be deallocated so that its memory is reclaimed.
In the newly-proposed schemes, we assume that this will be handled automatically by the 
Java garbage collection. In our analysis, we made the same assumption for all the competitors
we consider. However, Ben-David {\em et al.} describe in~\ref{BBF+21} how to manually reclaim memory
to make their scheme work also in languages that do not support automatic garbage collection. 
Specifically, BBF+ employs an implementation~\cite{ABW21}  of reference counting ~\cite{DM+01,HL+05} 
with amortized expected constant overhead on step complexity in order to 
reclaim (deallocate) all nodes that have been disconnected from the version lists. 
}






==> intro.tex <==
% !TEX root =  main.tex

\section{Introduction}
\label{sec:intro}

Multiversion concurrency control is widely used in database systems
\cite{Reed78,BG83,papadimitriou1984concurrency,HANAgc,neumann2015fast,Wu17},
transactional
memory~\cite{perelman2010maintaining,FC11,Perelman11,Kumar14,Keidar2015},
and shared data structures~\cite{BBB+20,FPR19,NHP21,WBBFRS21a}, mainly
for supporting complex queries (i.e., read-only transactions) in an atomic way, while update
operations are executed concurrently. 
This is usually achieved by maintaining a list of previous versions for each object.
Each version has a timestamp that indicates when the object was updated to that version.
Queries get a
timestamp $t$ and 
traverse objects' {\em version lists},
returning the latest version at or before~$t$.
%\Guy{Shortened the above while still mentioning timestamps.}
% The version list of each object $O$ stores an element for each of $O$'s updates 
% which is a pair comprised of the updated value and the update timestamp. 
% The list is sorted (in descending order) based on its elements' timestamps. 
% A query can first read a timestamp $t$ and then for each object 
% it accesses, traverse the object's version list to find the first version whose timestamp 
% is smaller than or equal to $t$.

Multiversion garbage collection (MVGC) is the problem of removing and
collecting obsolete versions.  
\er{Suppose one version has timestamp $t_1$ and the next version has timestamp $t_2$.
The version with timestamp $t_1$ is \emph{needed} if there is an ongoing query whose
timestamp $t$ satisfies $t_1\leq t < t_2$, and \emph{obsolete} otherwise.
The very latest version is always needed.}
%In general, a version is \emph{needed}
%if it is the latest version or if there is an ongoing query
%with a timestamp between it and the next later version, and is \emph{obsolete}
%otherwise.  
Efficient MVGC is an important problem in multiversioning
systems~\cite{lu2013generic,bottcher2019scalable,HANAgc,BBF+21,FC11,neumann2015fast,kim2019mvrlu,NHP21,WBBFRS21a}, 
since keeping obsolete versions can lead to excessive space usage.
%significant space problems.
%In addition to being space efficient,
%an MVGC scheme should be lightweight enough to exhibit low time overhead.  
%A flurry of research~\cite{lu2013generic,bottcher2019scalable,BBF+21,Fra04,B15,HL+05,M04,B15,SBM21,HANAgc} 
%has been devoted in designing efficient garbage collection schemes.
%that are efficient, both in terms of space and time. 

%\Eric{I rearranged this paragraph to deal with referee's complaint that space efficiency principle did not appear (explicitly) in \cite{lu2013generic}, as we seemed to be saying}
From a theoretical perspective, Ben-David et al.~\cite{BBF+21} recently gave
a state-of-the-art MVGC technique (henceforth \bbf{}). It is a
wait-free scheme that maintains only a constant factor more versions
than needed and uses $O(1)$ steps on average per allocated version.
\er{It is based on a fundamental {\em space efficiency principle} for the design of 
MVGC algorithms, which requires that obsolete versions are removed from 
version lists and reclaimed.}
%\here{deleted "intermediate" in preceding sentence in response to a comment from Youla}
Simple MVGC algorithms, such as epoch-based
reclamation
(EBR)~\cite{FC11,neumann2015fast,kim2019mvrlu,NHP21,WBBFRS21a}, that
delay reclamation of versions until all active operations have
terminated, force the system to retain many obsolete {\em
  intermediate versions} between the oldest required version and the
current one.  They therefore violate the space efficiency principle,
but they can manage versions lists quickly and simply
%are fast and simple 
because they do not require removing versions from the
middle of a version list.
\er{The removal of intermediate versions was first achieved in \cite{lu2013generic}
and later in~\cite{BBF+21,bottcher2019scalable,HANAgc}.}
To accomplish this, \bbf{} defined a {\em range tracking} object 
to precisely identify obsolete versions without having to
traverse the whole list.

%\here{I modified previous sentence because it's not completely clear that EBR is fast--for
%example, if lists are very long and queries have to traverse them, it's not so fast.
%What is fast and simple is the management of the version lists.
%Do we mention somewhere the added benefit of removing intermediate nodes:  shortening version lists
%is good in workloads where queries may hold old timestamps?}

%and thus utilize very simple techniques for updating the version lists.  

\Eric{I rewrote following parag.  We were using Steam and STEAM to refer to \cite{bottcher2019scalable}, so I changed them to Steam (to match the original paper).}
From a practical perspective, B\"ottcher et al.~\cite{bottcher2019scalable} gave a MVGC algorithm called Steam. 
Steam traverses a version list 
each time a new version is added to it, removing any obsolete versions, including intermediate ones.
Their experiments showed that this can significantly improve space usage and throughput
compared to some previous MVGC methods in workloads with complex queries and frequent updates.
However, %theoretically
the algorithm has no theoretic time bounds and for $P$
processes only achieves an $O(PM)$ bound on the number of versions contained in $M$ version lists,
which is significantly worse than the bound for \bbf{}.  On the other hand, it is unclear whether
 \bbf{}  can be highly time-efficient in practice, as it uses  %given that it uses
%some quite complicated components.  
%For example it uses 
a sophisticated wait-free doubly-linked list implementation, which we call \TreeDL\ 
because it has an implicit tree  laid over it
to achieve its time bounds.
% I commented out the following to save space because we already mention the specific bound above
%allow safely splicing versions out of the middle of a version list in
%constant amortized time.

We study the efficiency of these algorithms in
practice by implementing them and comparing them in a single system.
%\here{Is this accurate? We don't actually compare BBF+ in our experiments}
Based on our experiments, we  developed two novel MVGC algorithms that
combine and extend techniques from both Steam and \bbf{} to provide
protocols that are as space-efficient as \bbf{} while achieving
time efficiency comparable to Steam (sometimes slightly better, sometimes
slightly worse).  These algorithms relax some of the worst-case time
guarantees of \bbf{} to improve time performance in the common case.
However, they maintain the strong worst-case space bounds proved
in~\cite{BBF+21}.  Our experimental analysis reveals the practical
merit of state-of-the-art techniques for MVGC algorithms.  However, it
shows that their performance  depends
significantly on the workload and that there is no clear winner that
always dominates for both time and space.

Starting from the state-of-the-art MVGC schemes
in~\cite{BBF+21,bottcher2019scalable}, we had to apply, combine,
simplify or extend  techniques to obtain the two new MVGC
protocols (as discussed in Section~\ref{sec:mvgc}).  Both use
the range tracking (\RTO) object from \bbf{} to precisely identify
obsolete versions. %\Guy{However our second  traverses
%    the whole list anyway.  Perhaps say `` ... ''.} 
For the first protocol, called
\RTDLGC, we develop a new and simpler doubly-linked list
implementation supporting removal from the middle of version lists
(see Section~\ref{sec:dll}). The implementation, called \DL\
(Practical Doubly-linked List), sacrifices the guarantee of
constant amortized time per operation and instead guarantees $O(c)$
amortized time, where $c$ is the number of concurrent removals of
consecutive list nodes.  
%In the worst case, $c$ can be as high
%as the number of processes, $P$.  
%\here{I think it can be higher than $P$, since we're talking about interval contention not point contention.}
%\Hao{I agree, so I removed the previous claim}
This choice was driven by
the experimental insight that removing chains of adjacent nodes
is very rare in practice: in our experiments the
average $c$ was no more than 1.6 across a wide variety of workloads. 
Experiments show the new, simpler list is significantly faster
than the 
constant-time list when $c$ is small.
%Furthermore, it maintains the same space bounds as the original.  
%\here{I took out a sentence about the list maintaining the same space bounds
%because the list itself isn't what yields the space bounds; it is how it
%is used by the MVGC scheme, and we've already mentioned in previous parag that we maintain space bounds}

Our second algorithm,  \RTSLGC, further improves practical
  performance for many common workloads, in which version lists tend
  to be very short, so that linear searches are reasonably efficient.
In this case, we use a singly-linked list, which requires less space (no back pointers) and less time for
updates due to fewer pointer changes.  GVM~\cite{lu2013generic},
Steam~\cite{bottcher2019scalable} and HANA~\cite{HANAgc} also rely on
this observation~\cite{bottcher2019scalable}.  We develop
(Section~\ref{sec:sll}) a singly-linked list implementation, called
\SL\ (Simple Singly-linked List), and use it to implement version
lists in \RTSLGC.  Our implementation is very simple.  Unlike those in
Steam and HANA it is lock-free, 
and unlike GVM, which is lock-free, it does not require any mark bits
on pointers.  Such mark bits require an extra level of indirection in
safe languages that does not allow directly marking pointers.
%\here{Should we say more about distinction between SSL and GVM?}

Our new list structures support sorted
lists with an append on one end, and deletes anywhere, and are likely of
independent interest. We give a  proof of correctness for both. 
%In contrast to Steam, our MVGC protocols do not lock version lists and thus they can be  
%used in multiversioning systems that are not based on locks,
%e.g.,~\cite{WBBFRS21a}. 
% Moreover, instead of scanning
% the entire list on every update (as Steam does), our MVGC protocols use a range-tracking object 
% (as \bbf\ does) % from \bbf{} 
% to decide which elements of the version lists can be reclaimed (see Sections~\ref{sec:related} and~\ref{sec:implem} for more details on range tracking). 
Combining  our two new lists with the range tracker of \cite{BBF+21}
significantly improves space in many workloads over previous
 MVGC schemes. In particular, the range tracker 
identifies
an appropriate element in the list  to remove (in \RTDLGC) or a list  to traverse and collect (in \RTSLGC)
more accurately
than traversing a list on every update as in Steam or traversing lists with background threads
as in HANA and GVM.

In our experiments (Section~\ref{sec:experiments}), we implemented and studied several 
schemes: an optimized variant of Steam \cite{bottcher2019scalable} we developed using \SL, \bbf{}~\cite{BBF+21},
%\here{ER:Do we really have the original Steam? I thought it required locks.  Maybe "designed" is too strong.  "Optimized"?  "Developed"?}
%\here{Do we have experimental results on the original BBF+? }
%\Hao{We have experimental results for BBF+ but not original Steam as it would require taking locks and doesn't seem suitable for our use case. I editted the previous sentence according to the above comments.}
an epoch-based collector~\cite{WBBFRS21a}, and our new MVGC protocols.
%The experimental analysis sheds light on the reasons that this is so.
MVGC schemes encompass several mechanisms that may have a crucial effect on their time or space overhead.
We focussed on the following mechanisms that our experiments showed to have high impact on performance:
%(1) technique for deleting obsolete versions; 
(1) data structure for storing  versions 
and (2) how to choose when to traverse and compact a version list.
%\Eric{so that we don't do it when there is nothing to remove?}
%In the newly-proposed protocols, these three mechanisms have been designed so that they 
%respect the space- and time- efficiency principles. Even more, 

Our design decisions use several
insights that our experiments revealed.
\youla{It would be nice if we were able to list some insights in Section 6, 
derived from the presented diagrams. }
%\here{ER: I commented out a phrase here}
%; we found these insights 
% interesting and we consider them  to be part of the contribution of the paper.
%(some of them were also observed in previous works~\cite{+++}):
%
%\Guy{I feel these points could possibly be moved to a conclusion.
%I now think there is enough contribution to the paper without enumerating
%them here, and I feel like we have already made many of these points.}
%\here{ER: I agree}
%\here{PF: If the story is still the same, then I am ok. If however, the new story is that there is no clear
%winner (even after considering the proposed protocols) then it may be good to have some of the insights we gained from our experimental analysis.  
%Otherwise, I think it is not clear what we achieve in the paper.}
%\begin{enumerate}
%\item 
As in previous work~\cite{bottcher2019scalable}, we saw that reclaiming intermediate versions 
 is essential for reducing memory overhead,
especially when there are long queries or oversubscription (i.e., when there are more threads than cores). 
We  observed that removing chains of consecutive nodes concurrently is highly unlikely, % in practice,
and 
linked lists are often quite short in common workloads. 
%\youla{It would be nice if we report some numbers, eg average
%size of version lists in different exepriments to support this claim. Also, how many consecutive nodes we %delete on average.}
%, % \here{evidence?} \Hao{it's small in some workloads, but gets large in others}, 
%so in some cases, paying a higher cost of traversing a singly-linked list
%can be a better design decision than employing an implementation of a doubly-linked list with high overheads. 
%\Hao{I believe this is mentioned earlier in the intro as well. Perhaps we can move some of the details there.}
%Furthermore, we saw that 
%\item Safely removing from the middle of a version list is expensive. Previous techniques such as
%locking the entire version list during remove (as in Steam~\cite{bottcher2019scalable} or Hana~\cite{HANAgc}) or requiring 
%logically marking a next pointer in deletion~\cite{lu2013generic,FR04} are prohibitively expensive. 
%\here{Do we have any evidence to back up the latter statement?}
%\Hao{Unfortunately, we don't have any evidence. I'm thinking of dropping this bullet point because it has been mentioned earlier.}
%\item 
%the cost
%of traversing and compacting a version list should be avoided, if the chance of finding obsolete versions to reclaim is small.
%\youla{Which experiment shows this? Refer to it explicitly here or repeat this claim in Section 6 when discussing the relevant experiment.}
%\Hao{I don't think any experiment shows this. The two MVGC schemes that compact version lists, STEAM+LF and SL-RT, both perform compact at approximately the same frequency, SL-RT just does a better job of identifying version lists with garbage in it. Perhaps we can say that the STEAM heuristic of compacting right after the update leaves around a lot of obsolete versions.}
\er{We also saw that MVGC schemes such as Steam can waste time traversing versions that
are unlikely to be removed.}
For example, if a new version is added while there are ongoing queries, 
 the old version will likely still be needed by a query. 
\er{\RTSLGC\ avoids this problem because the superseded version is passed to the range tracking object of \cite{BBF+21} and then removed from its version list later, after the range tracking object identifies it as obsolete.}
%\youla{Refer to this again later on,
%when describing \RTSLGC. Also, we may want to provide an experiment which will show the impact of 
%applying this.}
%\here{Remember to describe how this delay works later in paper}
%\here{PF: I suggest to move this in preliminaries.tex.}
%\item 
%\item If linked lists are used for storing versions, they should, ideally, implemented as singly-linked. 
%Algorithms in~\cite{} we have experimented with, which employ doubly-linked version lists, had significantly
%lower throughput due to the time and space needed to maintain the prev pointers.  
%\item 
%In \emph{nested} multiversion data structures (such as multiversion tree in our experiments) where version lists point to tree nodes which in turn point other version lists, precise garbage collection is even more important. Any imprecision gets amplified because each obsolete version that is still reachable could recursively keep alive other version lists which themselves contain obsolete versions.
%Therefore, 
We also saw that in some workloads, keeping twice as many nodes as necessary in the version list might lead to 8 times more space usage.\here{Doublecheck number.  Explain why?}
%This is because some nodes
%in the version list may have pointers which point to  other version lists. Failing to
%collect such nodes in a version list might recursively keep alive many nodes in other version lists. \Hao{I believe this goes in the experiments section. Too much detail for the introduction.}
Finally, we observed a vicious cycle:  %\Hao{new item:} 
keeping more versions slows queries down because they must traverse longer version lists, which in turn causes more timestamps to be reserved, so compactions keep even more versions in the lists. This behavior was reported for EBR-based schemes in~\cite{bottcher2019scalable},  but we observed it in other MVGC schemes too.

Many existing practical techniques are heavily intertwined with other parts of the multiversion
system they were designed for. A previous study~\cite{bottcher2019scalable} compares MVGC schemes in various database
systems (including~\cite{bottcher2019scalable,HANAgc,larson2013hekaton}) that
use different transaction management protocols.
For our experiments, we separated out the ideas related to
memory management and fix all other parameters to isolate the %performance 
impact of the MVGC techniques. 
We know of no previous comprehensive, apples-to-apples
comparison of MVGC techniques.  
% Commented out following sentence (redundant because next parag says it is a contribution of paper
%We consider this to be another contribution of the paper.

We summarize the paper's contributions as follows.
\begin{itemize}[leftmargin=3mm,labelwidth=0mm,labelsep=1mm,topsep=0mm]
\item Two novel MVGC algorithms that borrow and extend ideas from state-of-the-art 
space- and time-efficient MVGC schemes.
%, exhibiting the benefits of both worlds. 
% commented out because it is not clear what worlds refers to, and next sentence makes point more clearly
The new algorithms maintain the strong worst-case space bounds provided by \bbf~\cite{BBF+21},
while achieving throughput comparable to Steam~\cite{bottcher2019scalable} in most cases.
\Hao{TODO: add numbers showing the two new algorithms have good space usage after writing up experiments section.}
\item An experimental analysis that {\em fairly} compares existing state-of-the-art 
MVGC schemes \er{by applying them all to the same data structures.
This sheds light on the practical merit of the schemes, and the reasons that no
%\here{should "none of the previously existing" be changed to "no"?  Current phrasing
%suggests no previous MVGC scheme dominates, but one of our new MVGC schemes does dominate}
%\Hao{I agree with this change, but we have to also make our new scheme sound good experimentally. I'll think about this some more.}
single }MVGC approach is a clear winner in terms of both space and time.
%\youla{Unclear, whether we cover this in a sufficient way in Section 6.}
\item Several insights, 
\Eric{If there is time, perhaps add something to Sec 6 to justify this bullet.}
which together with the space efficiency principle
%\Guy{Do we  still have two principles?},
can drive the design of new MVGC schemes, as they have for our new  schemes.
\item A new bounded-time doubly-linked list implementation \DL\ 
that exhibits good performance when used for MVGC,
and may be useful elsewhere. 
\item A new simple singly-linked list implementation \SL\ that is suitable for MVGC
and has better throughput than \DL. % in this setting.
%\Eric{Can we really make such a categorical statement?}
\end{itemize}




==> introduction.tex <==
%!TEX root = main.tex

\section{Introduction}

% rough notes:
%Having theoretical space (or time) bounds makes it robust to inputs and schedules. It ensures that space usage is low in all cases. This is why Epoch and Steam have bad cases whereas ours does not. Ours provides consistent performance across all workloads.

%Guy's comments: There are several existing approaches... however, all of these either have very weak or no bounds at all on either space or time. 
%Recent work has given much tighter bounds, but might not be practical.
%In this paper, we develop a new algorithm, which combines some of the ideas from the practical approaches and the theoretical paper.
%We maintain the space bounds from the theoretical paper, which gives us much better space usage than the other practical systems, and we maintain most of the time bounds, except in the doubly linked list.

%Time bound theorem: If $p$ processes are delete $p$ consecutive elements of a list, then the amortized cost is $p$.
%Parameterize time bounds with the maximum num of consecutive deletes.

%Guy's comment: We also devise a new algorithm for splicing out of a linked list (the one with linear time deletes). It's a lot simpler than all the ones that allow insertions and also simpler than our DISC. Trade-off where we sacrifice a bit of theoretical bounds for better time performance in practice.

%What's the take away? What insights can future people take away from this work.

%Youla's comments, there are practical work and theoretical work... the goal is to merge these two worlds. Combined scheme that has not so bad space overhead or 

%We came up with the new scheme which has the nice properties. To do this, we go through an experimental analysis which is comprehensive.
%By using both the theoretical and the practical scheme, we come up with these insights.

%these theory papers enjoy good space properties, but there are other papers that are more practical

%in order to get the new scheme we had to go on a journey. and along the journey this is what we learned.

%starting from this theoretical scheme, experiments showed that this and that are expensive.
%So we came up with ways to avoid it.

%We found out what the expensive components of the theoretical schemes and how to replace them.


Multiversion garbage collection (MVGC) is an important problem that has been identified as a bottleneck in real world database systems~\cite{bottcher2019scalable}.
Existing practical techniques either (1) have background threads periodically scan the version lists, looking for obsolete versions to collect, (2) use some variant of EBR to delay the reclamation of versions until all active multipoint operations have terminated, or (3) scan and compactify the entire version list whenever a new version is added to it.
Importantly, all of these technique either have very weak theoretical guarantees or none at all.
% Guy: add examples of how bad previous space bounds is
As a result, they often have bad time/space overheads in certain worst case inputs/executions.
Recently, a theoretical efficient algorithm has been developed which provides much tighter bounds on time and space~\cite{arxiv}, however it not known if it is practical.
% Notes from meeting: The fact that you have good theory bounds, doesn't necessarily mean that it has good practical performance. In practice, we verify that the theoretical algorithm has good space complexity, but not time. By investingating the reasons, we found that the limitations where x y, z. and we had to find 

In this paper, we develop two new MVGC algorithms, which combines ideas from the practical approaches and the theoretical paper.
Our first algorithm relaxes some of the worst-case guarantees of the theoretical paper to significantly improve its performance in the common case.
In particular, rather than supporting amortized constant time removals from version lists, we devise a simpler algorithm which takes amortized $O(c)$ time to perform this step, where $c$ is the number of concurrent removals of consecutive nodes in the list.
In the worst case, $c$ can be as high as the number of processes, $P$, however in practice, removing chains of adjacent nodes concurrently is very unlikely, so $c$ is usually no more than 2.
Our second algorithm further improves practical performance, but provides even weaker bounds on time.
It relies on the fact that version lists tend to be short in most workloads and therefore searching for a node from the head of the list is fast.
Many existing practical approaches also rely on this observation~\cite{bottcher2019scalable}.
The advantage of the second algorithm is that it is able to represent version lists using singly- rather than doubly-linked lists, which saves time when splicing in and out nodes.
Both algorithms maintain the strong wrost-case space bounds proven in~\cite{arxiv}, and as a result, has low space usage in practice across the variety of workloads we ran.
We measured the theoretical minimum memory usage assuming a precise garbage collector and showed that our two new algorithm are very close to this theoretical minimum in all workloads, as predicted by the theory.
In contrast, previous practical approaches have certain bad workload where they performed poorly.
Furthermore, the throughput of our most optimized algorithm is competitive with previous practical approaches.

Many of the existing practical techniques are heavily intertwined with other parts of the multiversion system they were designed for, so one of the contributions of this paper is separating out the ideas related to memory management.
To the best of our knowledge, there has not been any comprehensive, apples-to-apples comparison of these techniques.
For example, an existing study~\cite{bottcher2019scalable} compares MVGC in various database systems including Steam\footnote{To distinguish between the database system and the GC technique, I will use SteamGC to refer specifically to the GC technique.}, Hana, and Hekaton, however, these database systems also use different transaction management protocols.
In our experimental comparison, we fix all other variables to isolate the performance impact of the MVGC techniques.
We show that the performance of existing techniques depend heavily on the workload and that there is no clear winner.
For example, in some workloads, EBR might use significantly less memory compared to SteamGC (Figures~\ref{fig:batch-2-oversub} and ~\ref{fig:batch-2-undersub}), but on others it is the complete opposite (Figure~\ref{fig:batch-64-undersub}).
We also show the value of theoretical bounds because it ensures consistent good performance regardless of the workload.

All our experiments are performed in Java.
% Note: try enabling the Java garbage collector to see how that affects the times. I would assume that more precise MVGC algorithms benefit more from this.
Note that Java's garbage collector on its own does not solve the MVGC problem because old versions are still reachable via the version lists.
%The MVGC algorithm is responsible for identifying unneeded versions and making them available to be collected by the garbage collector.



\paragraph{Insights from Experiments.}

\begin{itemize}
	\item The ability to reclaim ``gaps'' in the version list is essential for reducing memory overhead in practice, especially when there are long operations or more threads than cpus. (This has been observed before) (guy's suggestion: make this no longer an insight and say "as consistent with the work on steam, we found that reclaiming gaps...")
	\item Version lists should ideally be singly linked. All the doubly-linked version lists we ran had significantly lower throughput due to the time and space needed to maintain the back pointers. (haven't seen this pointed out before, but it sounds obvious enough.)
	\item Safely removing from the middle of a version list is expensive. Previous work either locks the entire version list during remove (Steam, Hana) or requires logically marking a node for deletion. Our observation is that both are not required because the remove operation need not be safe.
	If we simply using a CAS to shortcut out the desired node, the worst that can happen is that the node might reappear in the version list due to a concurrent \texttt{remove}.
	This is fine in the MVGC setting as long as some operation eventually tries to remove this node again.	
	(this insight might be more interesting that the previous two.) We used this to develop SteamGCours, which is significantly faster than SteamGC.
	\item In some workloads, keeping a factor of 2 more nodes than necessary in the version list might lead to a factor of ~10 more space usage (Figures~\ref{fig:batch-2-oversub} and ~\ref{fig:batch-2-undersub}). For example in our snapshottable tree, each node in the version list also has left and right pointers which point to two other version lists. So failing to collect one node in a version list might recursively keep alive many other version lists.
	\item If a new version is added while there are ongoing range queries, then chances are, the old version will still be needed by one of those range queries. Therefore, we do not want to scan and compact the version list as soon as it is updated (like in Steam), but rather after some delay. 
\end{itemize}

%Using these insights, we developed a new technique which gets the best of both worlds (in terms of space) between EBR and SteamGCours, while being competitive in terms of time.
%We measured the theoretical minimum memory usage assuming a precise garbage collector (not shown in graphs just yet) and showed that our new algorithm is very close to this theoretical minimum in all workloads.

%The key idea is to... 

==> mvgc-techniques.tex <==
% !TEX root =  main.tex

\section{MVGC Implementations}
\label{sec:implem}

We show how to use the singly- and doubly-linked list algorithms in the previous sections to improve two existing MVGC techniques (steam and BBF+) as well as develop a new one.

\subsection{Lock-free Steam}

%Steam works in transactional system, where each thread manages a disjoint set of transactions.
%Each thread $p$ keeps track of the timestamps of the transactions it manages in a local list
%and announces the current timestamp 
In Steam~\cite{bottcher2019scalable}, version lists are singly-linked lists sorted in decreasing order, 
based on the timestamps of the versions.
A new version is added in the version list of an object, every time the object is updated. 
Then, $p$ traverses the version list that it has just updated, 
and compacts it by deleting all versions that are not needed by any currently active transaction. 
To implement compaction, the  timestamps announced by active queries are collected and
sorted, in decreasing order, by $p$ before starting the traversal of an updated version list. 
Steam supports transactions by using locks to apply multiple updates in an atomic way. 
Compaction of version lists is piggy-backed in transactions' processing 
(as part of objects' updates), so a version list is locked 
when its compaction takes place. 
It follows that Steam is blocking. 

Given that compaction of a version list is performed every time 
a new version is added in it and assuming that announced timestamps are collected every time
a compaction occurs, the size of any version list is $O(P)$ (recall that $P$ is the number of processes).
We have implemented a lock-free version of Steam, called \texttt{SteamLF}, 
by employing the lock-free compaction algorithm presented in Section~\ref{sec:sll}. 
Specifically, \texttt{SteamLF} implements and manipulates each version list using the 
lock-free singly-linked list implementations presented in Figure~\ref{alg:singly-linked-list-compact}. 
Apart from this change, \texttt{SteamLF} works in the same way as Steam. 
Invariant~\ref{} implies that \texttt{SteamLF} maintains the $O(P)$ space bound of Steam. 

\here{PF: If the space bound of ssl does not hold, we need to update the last sentence above.
It seems to me that the bound is tighter than O(P), it is O(\# of needed versions).}

\here{PF: collect versus scan versus list traverse?}

\ignore{
\begin{itemize}

	\item Recall that Steam compacts a version list whenever a new version is added to it.
	\item The original Steam paper locks the version list before compacting, we can make this lock-free using our lock-free compact from Section~\ref{sec:sll}. We call the resulting algorithm \texttt{SteamLF}.
	\item If the announcement array is scanned on every compact, then this would maintain the space bounds of Steam (i.e. each version list has length at most $O(P)$).
\end{itemize}
}

\subsection{Practical BBF+}
\label{sec:pBBF+}

We propose a more practical version of BBF+, called PBBF+, 
which employs RangeTracker~\cite{BBF+21}, the linerizable implementation of a range-tracking object used by BBF+, 
but replaces the doubly-linked list implementation of BBF+
with the doubly-linked list implementation described in Section~\ref{sec:dll}. 
We provide more details below, starting with a description of  RangeTracker.
%
%We first provide a more detailed description of RangeTracker. 

%{\em RangeTracker}. 
A range-tracking object supports three operations, 1) \announce\ to announce a new timestamp, 2) \unannounce\ 
to declare that a previous announcement is no longer active, and 3) \deprecate, which 
declares that a version $v$ of an object is no longer the object's current version and 
identifies a set of unneeded nodes that can be safely disconnected from the object's version list.   
Every time a version $v$ ceases from being the current, 
\deprecate\ is invoked to declare that $v$ is no longer current and compact the version list $v$ resides. 

RangeTracker ensures that, in the worst case, \announce\ and \unannounce\ take $O(1)$ steps, 
and \deprecate\ takes $O(P\log P)$ steps but its amortized step complexity is $O(1)$. 
Operations \announce\ and \unannounce\ use a destination object~\cite{BW20a} to announce and unannounce 
timestamps in an announcement array $Ann$ in $O(1)$ steps.
To achieve its bounds, operation \deprecate\ works as follows. 
When a thread $p$
calls \deprecate\ for some version $v$, $v$ is appended in a local list where $p$ stores
objects it has deprecated; the list is sorted in decreasing order of timestamps of the deprecated objects it contains. 
If the size of $p$'s local list becomes $P\log P$ (where $P$ is the number of processes), a {\em flush phase} is performed: 
$p$'s  list is appended in a shared queue $Q$ containing such lists; then, two lists are extracted from $Q$,
their contents are merged and they are compared against a sorted version of $Ann$ to determine those versions
that are still needed, which are appended again into $Q$, and the set of the unneeded nodes that will be returned. 
This process is done with care, so that a flush phase requires $O(P\log P)$ steps and is perfrormed once
for every $O(P\log P)$ calls to \deprecate. Moreover, it is proved in~\cite{BW20a},
that RangeTracker satisfies the space bound of $O(H + P^2\log P)$, where $H$ is the number of needed versions. 

\y{
Experiments showed that employing RangeTracker results in some space overhead in practice. To reduce constants
in the space bound it ensures, we have implemented the following optimizations:
\begin{itemize}
\item pop a constant number of queues bigger than two every time we execute the flush phase. \here{PF: Have we implemeneted this optimization? Is it worth-mentioning?}
\item before we push a local queue in the global queue, compact the list, i.e., try to remove those versions in it that are already marked as unneeded. 
These techniques may reduce the space overhead imposed by RangeTracker without violating the space and time bounds it ensures. 
\end{itemize}

Another optimization we have discussed is to ocassionally, pick a random version list to go through and compact. 
Have we tried this? Shall we refer to it?
}

{\em Lock-Free Doubly-Linked List}. We first present some of the details of TreeLL,
as it served as the starting point for designing DLL. We mainly focus on the implementation 
of \remove, as the rest of the routines are much simpler and do not impose any major difficulties.
%BBF+-DLL (as DLL) supports the operations, \tryAppend, which appends a node at the
%head of the list, \find, which searches for the first node in the list that has a timestamp 
%smaller than or equal to its argument, and \remove, which takes a pointer to a node as an argument 
%and splices the node out from the list. 
TreeLL supports the operations, \tryAppend, \find, and \remove, which have similar
functionality as the corresponding operations of DLL (the implementation in Section~\ref{sec:dll}). 
To remove a node, TreeLL marks it for deletion and then splices it out from the list. 
The major drives behind the design of \remove\ in PPB+-DLL are to avoid
list inconsistencies when deleting subsequent nodes, while ensuring 
the desired theoretical bounds.

TreeLL embeds a conceptual priority tree in the linked list
whose inorder traversal results in an ordered sequence of the list nodes.
TreeLL owns its name to this technique of organizing removals based on a priority tree.
%(this idea has been proposed in~\cite{++} for parallel list contraction). 
As long as deletions take place at the leaves of the tree (i.e., as long as 
a node is deleted only after all its descendants in the tree have been deleted), 
no two subsequent nodes of the tree are deleted concurrently, so 
consistency is ensured. However, some leaves may be still needed for answering queries.
Such leaves may block progress of removals and result in higher space bounds. 
To solve this problem, PBF+-DLL uses a helping mechanism 
which allows marked nodes that may have an unmarked neighbor to be spliced out (in some cases). 
This is done with much care, using two special helping routines, namely \spliceUnmarkedLeft, and \spliceUnmarkedRight, 
which ensure that consistency of the list is maintained. Moreover, this design 
preserves the desired bounds. 
Specifically, TreeLL ensures that 
at most  $2(L-R) + O(P\log L_{max})$ nodes remain in the version lists in an execution
containing a total of $L$ appends and $R$ removes, and at most $L_{max}$ appends 
on a single version list. It also ensures that 
\tryAppend\ and \getHead\ 
take $O(1)$ steps, and the amortized  number of steps for \remove\ is $O(1)$.

\spliceUnmarkedLeft\ and \spliceUnmarkedRight\ are pretty complicated, and  
experiments illustrated that they are pretty heavy in terms of performance. 
To come up with DLL, we first tried deactivating 
\texttt{spliceUmarkedLeft} and \texttt{spliceUnmarkedRight}, thus compromising
the space bound that TreeLL exhibits. 
Unfortunately, experiments showed that this simple solution ended up increasing 
space usage significantly (resulting in version lists that were on average twice 
as long as needed). DLL is thus a new proposed design, which avoids this space cost,
maintaining the good space bounds from~\cite{BBF+21}\here{PF: Is the space bound
the same for both DLL algorithms, the one in Section~\ref{sec:DLL} and TreeLL?}. 

\here{PF: We need to say more here.}
In terms of time, DLL ensures that \tryAppend\ and \getHead\ 
maintain the $O(1)$ bound of TreeLL, but the amortized  number of steps for \remove\ is $O(c)$,
where $c$ is the number of concurrent removals of consecutive nodes in the list.
Experiments showed that $c$ is usually a small constant; specifically, 
we saw that each \remove\ visits less than $3.6$ nodes on average \here{PF: Hao, please check if this number
is correct.}. This implies that, from a practical perspective, relaxing the time bound for \remove\
to $O(c)$ is a good compromise. 

\begin{theorem}

\end{theorem}


%Next, we tried a more practically efficient doubly linked list algorithm (without the theoretical guarantees of the one presented in the DISC paper) shown in Algorithm~\ref{alg:doubly-linked-list}, and that speed things up a little bit.


\ignore{

\paragraph{{\em \bf BBF+.}}
We start by providing an overview of BBF+. 
BBF+ assumes that every query sets a timestamp (i.e., it records an increasing integer in a global shared variable) 
at the beginning of its execution. Every update operation starts by reading the current timestamp 
(stored in this global variable) and uses it to stamp all the updates it performs. The previous value 
of an updated object (and its timestamp) are appended in the object's version list. 
After setting a new timestamp, a process executing a query proceeds to read the objects
that are necessary for computing its response. To do so in a consistent way, 
it traverses the version list of each such object and collects the first version it finds there 
with a timestamp that is smaller than or equal to the timestamp that the query set. 

Garbage collection in BBF+ employs the following two major components: 1) a {\em range tracking object},
which stores a set of versions and identifies those that are no longer needed, and 
2) a lock-free {\em doubly-linked list} to implement each object's version list, 
which supports an operation \Remove\ for disconnecting the unneeded versions. 
We briefly discuss each of these mechanisms below.

\paragraph{{\em \bf Practical Version of BBF+.}}
}


\subsection{SPAA2}
\Hao{TODO: pick better names for our algorithms.}

SSL-MVGC

\begin{itemize}
\item A combination of BBF+ and SteamLF. The high-level idea is to use the range tracker from BBF+ to identify version lists with garbage in them, 
and then compact any version list that is returned by the range tracker.
\item This allows us to use a singly linked list, which saves space (no need for back pointers), and time, 
but the disadvantage is having to re-traverse from the head when removing nodes.
\item  More precise description of algorithm: if $h_{o}$ is the current head of a version list $L$, 
whenever we append a new head $h_{n}$ to $L$, we \texttt{deprecate} the triplet $(L, h_{o}.ts, h_{n}.ts)$, where $[h_{o}.ts, h_{n}.ts)$ defines an interval of time. 
This \texttt{deprecate} operation returns a (possibly empty) list of previously deprecated triplets 
who's time intervals are no longer reserved. We call \texttt{compact} on each version list in the triplets 
that are returned. Note that a version list could be \texttt{deprecate}d multiple times, 
each time associated with a different time interval, so we remove duplicates before calling compact.
\item If a triplet $(L, h_{o}.ts, h_{n}.ts)$ is returned by \texttt{deprecate} and later \texttt{compact(L)} is called, 
then $h_{o}$ is guaranteed to not be reachable in $L$ and will never become reachable again. 
Note that $h_{o}$ might have been removed by some earlier compact on $L$, so this call to \texttt{compact(L)} might end up finding no nodes to remove.
\item Brief justification of why space bounds of BBF+ are maintained.
\item Theoretical time bounds can be bad if version lists get long.
\item TODO (Hao): finalize the set of optimization in the experiments and describe them here
\end{itemize}


Finally, we tried making the linked lists singly linked (further weakening its theoretical guarantees), 
and this had the best throughput out of all these variations (while at the same time maintaining the low space overhead of the original algorithm).
Since we no longer maintain back pointers, deleting from the middle of the list requires re-traversing the list from the head pointer.
This turns out to not be that expensive in our experiments because the version lists tend to be short.
The high-level idea behind this algorithm is to use our range tracker to identify version lists with garbage in them, and then scan\&compact any version list that is returned by the range tracker.



\ignore{
\noindent 
{\bf Memory Reclamation for nodes deleted from version lists.} 
As soon as a node is sliced out from a version list, it can be deallocated so that its memory is reclaimed.
In the newly-proposed schemes, we assume that this will be handled automatically by the 
Java garbage collection. In our analysis, we made the same assumption for all the competitors
we consider. However, Ben-David {\em et al.} describe in~\ref{BBF+21} how to manually reclaim memory
to make their scheme work also in languages that do not support automatic garbage collection. 
Specifically, BBF+ employs an implementation~\cite{ABW21}  of reference counting ~\cite{DM+01,HL+05} 
with amortized expected constant overhead on step complexity in order to 
reclaim (deallocate) all nodes that have been disconnected from the version lists. 
}






==> new-code.tex <==
\begin{verbatim}

void compact(List<int> sortedAnn, int scanTS, Node *head)
   sortedAnn.appendFront(-1); 
   int i = sortedAnn.size()-1;

   Node *curr = head;
   
   while (curr->ts > scanTS) curr  = curr->left; 
   
   Node *Left = curr->left;
   Node *oldLeft = Left; 
   
    while (Left != NULL) { 
	while (sortedAnn[i] >= curr->ts) i--;
	while (sortedAnn[i] < Left->ts) Left = Left->left;
	if (Left != oldLeft) {
	   while (!CAS(&(curr->left), oldLeft, Left)) {
		oldLeft = curr->left; 
		if (oldLeft->ts <= Left->ts)) break; 
	   }  
	}
	curr = curr->left;
	Left = curr->left;
	OldLeft = Left; 
   }
}
\end{verbatim}




==> optimization-notes.tex <==
% !TEX root =  main.tex



\subsection{Optimizations}
\label{sec:opt-notes}

\subsubsection{Reserving Timestamps} Both BBF+ and our singly-linked list compaction algorithm from Section~\ref{sec:sll} use atomic copy (a primitive which allows us to atomically read from one memory location and write to another) to announce timestamps in a wait-free manner. Instead, in our experiments, we use a lighter-weight lock-free scheme for announcing timestamps which consist of (A1) reading the current timestamp, (A2) announcing it, and (A3) checking if the current timestamp is still equal to what we announced and going back to step A1 if does not.
This means that a process scanning the announcement array might see a very old timestamp get announced, which breaks the monotonicity property required for the correctness of our singly linked list.
We fixed this by having all processes work on updating a global scan of the announcement array as described in Section~\ref{sec:sll} \Hao{I have not checked that this appears in Section~\ref{sec:sll}, but we talked about adding it there in the meeting.}.
When reading the announcement array, we ignore any timestamp that (1) is smaller than the timestamp at which the current global scan was taken and (2) does not appear in the current global scan.
This is safe because any announced timestamp satisfying these two conditions will fail the check in step A3, and not be used.
This change to how we scan announcement arrays ensures that the global scan satisfies the monotonicity property required by our singly linked list.
This announcement/scanning algorithm is used by LockFreeSteam, BBF+, and PBBF+, and SLL-MVGC.

%\subsection{SLL-MVGC} 
%
%It was crucial to compact the entire version list whenever one gets returned by the range tracking data structure (as opposed to just removing the 1 node associated with the returned range). This is because version lists can sometimes get extremely long, so traversing the list during remove() becomes small. Note that this is not necessary in SPAA1 because remove operation jump directly to the node. Collecting all the nodes in a version list also makes SPAA2 have less memory usage in some cases.

\ignore{
\subsubsection{Range Tracker}

There were several space and time trade-offs to consider when implementing the range tracker. A crucial one is how often to remove batches of nodes from the global queue. For their theory bounds, the BBF+ paper pops $c=2$ batches every time a batch is pushed onto the queue. Their bounds would still hold for any constant $c>1$.
They note that higher $c$ leads to smaller constants in the space bound, but higher constants in the time bound.
In general, when tuning these parameters, we prioritized maximizing throughput, and then reducing space usage as much as possible.
We found that for all range-tracker based algorithms, choosing $c=1.5$ lead to good results, which means we alternate between popping 1 batch and popping 2 batches.
Another parameter is how many nodes to accumulate locally before pushing onto the global queue, and we found that 4 times the number of threads was the smallest we could set this parameter while maintaining good throughput.


\subsubsection{Lock-free Steam} Instead of re-scanning the announcement array on every compact(), each thread updates the global scan of the announcement array only if it is more than 1ms old. 
The original paper suggested scanning every 50ms, but that was too slow for the workloads in our experiments where update throughput can be very high (up to 40K updates per ms).
}


==> techniques.tex <==
%!TEX root = main.tex

\section{MVGC techniques}

\subsection{Background Threads}

One solution to the MVGC problem (used by HANA~\cite{HANAgc} and GMV~\cite{lu2013generic}) is to have background threads that periodically scan all the version lists and compactify them.
The issue is that the number of GC threads might be hard to tune if update frequencies fluctuate frequently.

All of the later methods in this section do not use background threads and instead each updating thread performs some work towards the cleanup.
This way, the number of garbage collection steps scales naturally with the number of updates.

\subsection{EBR-based techniques}

Another solution is to use Epoch-based techniques. These techniques are fast because they don't require removing from the middle of a version list and EBR is known to have low time overhead in the standard SMR setting.
Epoch-based techniques are used in Cicada~\cite{lim2017cicada}, snapshottable data structures~\cite{WBBFRS21a}, and a recent survey comparing various MVCC (multiversion concurrency control) implementations~\cite{Wu17}.

\subsection{Steam}

SteamGC scans and compacts a version list whenever a new version is added to it.
Compacting involves first scanning and sorting the announcement array and then merging it with the version list.
Scanning the announcement array on every update is too expensive so the authors suggest a heuristic where the announcement array is scanned at most once every 50ms.
We found that 1ms was a more reasonable delay in our experiments because our workloads have higher update throughput.
The list can still be compacted with this out-of-date scan, however it would not be as precise, since any version that is more recent than the scan cannot be collected.
%Rather than waiting a fixed amount of time between consecutive scans, we instead scan the announcement array whenever the version list we are compacting contains a timestamp greater than the timestamp at the start of our previous scan.
%In most cases, the previous scan is up-to-date enough and does not need to be updated.
We also applied an optimization for unlinking version nodes without locking.

\subsection{Range-Tracker Based}

We implemented several variations of the algorithm from our DISC paper~\cite{BBF+21}.
The algorithm described in the paper has extremely good space complexity in practice (achieving the best of both worlds between EBR and Steam), but also significant time overhead.
We tried several ways of reducing this time overhead.
First, we tried getting rid of the two most complex operations, \texttt{spliceUmarkedLeft} and \texttt{spliceUnmarkedRight}, but this ended up increasing space usage significantly (version lists were on average twice as long as needed).
Next, we tried a more practically efficient doubly linked list algorithm (without the theoretical guarantees of the one presented in the DISC paper) shown in Algorithm~\ref{alg:doubly-linked-list}, and that speed things up a little bit.
Finally, we tried making the linked lists singly linked (further weakening its theoretical guarantees), and this had the best throughput out of all these variations (while at the same time maintaining the low space overhead of the original algorithm).
Since we no longer maintain back pointers, deleting from the middle of the list requires re-traversing the list from the head pointer.
This turns out to not be that expensive in our experiments because the version lists tend to be short.
The high-level idea behind this algorithm is to use our range tracker to identify version lists with garbage in them, and then scan\&compact any version list that is returned by the range tracker.

\subsection{GMV}

improvements: have a shared queue to avoid redundant GC work.


add a hashtable 



